Stability and Dynamics of Many-Body Localized Systems Coupled to Small Bath

It is known that strong disorder in closed quantum systems leads to many-body localization (MBL), and that this quantum phase can be destroyed by coupling to an infinitely large Markovian environment. However, the stability of the MBL phase is less clear when the system and environment are of finite and comparable size. Here, we study the stability and eventual localization properties of a disordered Heisenberg spin chain coupled to a finite environment, and extensively explore the effects of environment disorder, geometry, initial state and system-bath coupling strength. By studying the non-equilibrium dynamics and the eventual steady-state properties of different initial states, our numerical results indicate that in most cases, the system retains its localization properties despite the coupling to the finite environment, albeit to a reduced extent. However, in cases where the system and environment is strongly coupled in the ladder configuration, the eventual localization properties are highly dependent on the initial state, and could lead to either thermalization or localization.

==> Backup.tex <==
\begin{comment}
\begin{thebibliography}{}

\bibitem{abanin2019colloquium,
  title={Colloquium: Many-body localization, thermalization, and entanglement},
  author={Abanin, Dmitry A and Altman, Ehud and Bloch, Immanuel and Serbyn, Maksym},
  journal={Reviews of Modern Physics},
  volume={91},
  number={2},
  pages={021001},
  year={2019},
  publisher={APS}
}

\bibitem{MBL_dissipation}
Levi, Emanuele and Heyl, Markus and Lesanovsky, Igor and Garrahan, Juan P.,
Robustness of Many-Body Localization in the Presence of Dissipation
\href{https://link.aps.org/doi/10.1103/PhysRevLett.116.237203}{Phys. Rev. Lett., \textbf{116}, 237203 (2016)}

\bibitem{MBL_small_bath}
Hyatt, Katharine and Garrison, James R. and Potter, Andrew C. and Bauer, Bela,
Many-body localization in the presence of a small bath,
\href{https://link.aps.org/doi/10.1103/PhysRevB.95.035132}{Phys. Rev. B, \textbf{95}, 035132 (2017)}.

\bibitem{marino2018many}
J. Marino and R. M. Nandkishore,
Many-body localization proximity effects in platforms of coupled spins and bosons

\bibitem{serbyn2013local}
M. Serbyn, Papi\ifmmode \acute{c}\else \'{c}\fi{}, Z. and Abanin, Dmitry A., Local Conservation Laws and the Structure of the Many-Body Localized States,
\href{https://doi.org/10.1103/PhysRevLett.111.127201}{Phys. Rev. Lett., \textbf{111}, 127201 (2013)}.

\bibitem{huse2014phenomenology}
David A. Huse, Rahul Nandkishore, and Vadim Oganesyan, Phenomenology of fully many-body-localized systems, \href{https://link.aps.org/doi/10.1103/PhysRevB.90.174202}{Phys. Rev. B, \textbf{90}, 174202 (2014)}

\bibitem{programmable_random}
Smith, J., A. Lee, P. Richerme, B. Neyenhuis, P. W. Hess, P. Hauke,
M. Heyl, D. A. Huse, and C. Monroe, Many-body localization in a quantum simulator with programmable random disorder, \href{https://doi.org/10.1038/nphys3783}{Nat. Phys. \textbf{12}, 907 (2016)}

\bibitem{hamming}
P. Hauke and M. Heyl, 
Many-body localization and quantum ergodicity in disordered long-range Ising models,
Phys. Rev. B 92, 134204 (2015).

\bibitem{experiment_2d}
Choi, Jae-yoon and Hild, Sebastian and Zeiher, Johannes and Schau{\ss}, Peter and Rubio-Abadal, Antonio and Yefsah, Tarik and Khemani, Vedika and Huse, David A. and Bloch, Immanuel and Gross, Christian,
Exploring the many-body localization transition in two dimensions.

\bibitem{supercond_q}
Emulating Many-Body Localization with a Superconducting Quantum Processor, PRL

\bibitem{spin_ladder}
Pierre Bouillot, Corinna Kollath, Andreas M. Läuchli, Mikhail Zvonarev, Benedikt Thielemann, Christian Rüegg, Edmond Orignac, Roberta Citro, Martin Klanjšek, Claude Berthier, Mladen Horvatić, and Thierry Giamarchi,
Statics and dynamics of weakly coupled antiferromagnetic spin-1/2 ladders in a magnetic field,
Phys. Rev. B 83, 054407

\bibitem{dissipation1}
Emanuele Levi, Markus Heyl, Igor Lesanovsky, and Juan P. Garrahan
Robustness of many-body localization in the presence of dissipation

\bibitem{dissipation2}
Benjamin Everest, Igor Lesanovsky, Juan P. Garrahan, Emanuele Levi,
Role of interactions in a dissipative many-body localized system



\end{thebibliography}
\end{comment}

==> Introduction.tex <==
\section{Introduction}\label{sect:intro}


